Beyond Mahalanobis-Based Scores for Textual OOD Detection

Deep learning methods have boosted the adoption of NLP systems in real-life applications. However, they turn out to be vulnerable to distribution shifts over time which may cause severe dysfunctions in production systems, urging practitioners to develop tools to detect out-of-distribution (OOD) samples through the lens of the neural network. In this paper, we introduce TRUSTED, a new OOD detector for classifiers based on Transformer architectures that meets operational requirements: it is unsupervised and fast to compute. The efficiency of TRUSTED relies on the fruitful idea that all hidden layers carry relevant information to detect OOD examples. Based on this, for a given input, TRUSTED consists in (i) aggregating this information and (ii) computing a similarity score by exploiting the training distribution, leveraging the powerful concept of data depth. Our extensive numerical experiments involve 51k model configurations, including various checkpoints, seeds, and datasets, and demonstrate that TRUSTED achieves state-of-the-art performances. In particular, it improves previous AUROC over 3 points.

==> all_combinations.tex <==
\begin{longtable}{llllrrrrrrrrrrrrrr} \toprule      &       &     &                     &     error &       fpr &   aupr in &  aupr out &     auroc &   checkpoint &       seeds &  error.std &   fpr.std &  aupr in.std &  aupr out.std &  auroc.std &  checkpoint.std &   seeds.std \\ in ds & out ds & tech & layer &           &           &           &           &           &              &             &            &           &              &               &            &                 &             \\ \midrule 20ng & imdb & energy & energy predictions &  0.146162 &  0.153490 &  0.764157 &  0.996532 &  0.967282 &  7542.857143 &  277.500000 &   0.166309 &  0.178922 &     0.085338 &      0.005352 &   0.029217 &     6634.747605 &  134.626779 \\      &       & int w halfs pace unn & pw 1 &  0.068192 &  0.069606 &  0.911068 &  0.997827 &  0.982408 &  7542.857143 &  277.500000 &   0.053757 &  0.057832 &     0.058313 &      0.001709 &   0.011156 &     6634.747605 &  134.626779 \\      &       & maha & pooled &  0.037417 &  0.036501 &  0.929375 &  0.999274 &  0.991443 &  7542.857143 &  277.500000 &   0.021739 &  0.023385 &     0.039719 &      0.000482 &   0.005167 &     6634.747605 &  134.626779 \\      &       & msp & softmax predictions &  0.200731 &  0.212198 &  0.719163 &  0.996177 &  0.957284 &  7542.857143 &  277.500000 &   0.069290 &  0.074545 &     0.078599 &      0.001249 &   0.012743 &     6634.747605 &  134.626779 \\      & mnli & energy & energy predictions &  0.204417 &  0.219365 &  0.752822 &  0.994618 &  0.954226 &  7542.857143 &  277.500000 &   0.119680 &  0.131232 &     0.067495 &      0.003394 &   0.020678 &     6634.747605 &  134.626779 \\      &       & int w halfs pace unn & pw 1 &  0.089673 &  0.093613 &  0.933360 &  0.997436 &  0.982345 &  7542.857143 &  277.500000 &   0.097212 &  0.106535 &     0.066260 &      0.002708 &   0.017817 &     6634.747605 &  134.626779 \\      &       & maha & pooled &  0.095902 &  0.100377 &  0.885202 &  0.997035 &  0.974388 &  7542.857143 &  277.500000 &   0.106500 &  0.116781 &     0.177196 &      0.004988 &   0.043998 &     6634.747605 &  134.626779 \\      &       & msp & softmax predictions &  0.319025 &  0.345035 &  0.686265 &  0.991773 &  0.929410 &  7542.857143 &  277.500000 &   0.082507 &  0.090470 &     0.067715 &      0.002329 &   0.019368 &     6634.747605 &  134.626779 \\      & multi30k & energy & energy predictions &  0.097593 &  0.134197 &  0.959214 &  0.975139 &  0.970115 &  7542.857143 &  277.500000 &   0.092614 &  0.161573 &     0.035761 &      0.031347 &   0.028204 &     6634.747605 &  134.626779 \\      &       & int w halfs pace unn & pw 1 &  0.034404 &  0.034253 &  0.991890 &  0.988164 &  0.991160 &  7542.857143 &  277.500000 &   0.037049 &  0.056539 &     0.009941 &      0.015280 &   0.010962 &     6634.747605 &  134.626779 \\      &       & maha & pooled &  0.051584 &  0.055625 &  0.980699 &  0.989389 &  0.986418 &  7542.857143 &  277.500000 &   0.060950 &  0.105214 &     0.057858 &      0.023337 &   0.033525 &     6634.747605 &  134.626779 \\      &       & msp & softmax predictions &  0.129513 &  0.189590 &  0.943104 &  0.967669 &  0.956992 &  7542.857143 &  277.500000 &   0.083445 &  0.145831 &     0.044634 &      0.026467 &   0.035107 &     6634.747605 &  134.626779 \\      & rte & energy & energy predictions &  0.235190 &  0.352582 &  0.847399 &  0.937657 &  0.903795 &  7776.119403 &  279.985075 &   0.082049 &  0.133901 &     0.046637 &      0.023771 &   0.026432 &     6687.439369 &  135.751834 \\      &       & int w halfs pace unn & pw 1 &  0.101691 &  0.135836 &  0.969786 &  0.978635 &  0.975078 &  7776.119403 &  279.985075 &   0.088755 &  0.143716 &     0.030524 &      0.022329 &   0.024700 &     6687.439369 &  135.751834 \\      &       & maha & pooled &  0.122186 &  0.168194 &  0.941890 &  0.974595 &  0.962085 &  7776.119403 &  279.985075 &   0.075780 &  0.123647 &     0.095613 &      0.028758 &   0.048414 &     6687.439369 &  135.751834 \\      &       & msp & softmax predictions &  0.330340 &  0.507866 &  0.801979 &  0.908081 &  0.863150 &  7776.119403 &  279.985075 &   0.066339 &  0.108252 &     0.050694 &      0.024172 &   0.038106 &     6687.439369 &  135.751834 \\      & sst2 & energy & energy predictions &  0.085695 &  0.124045 &  0.978658 &  0.971486 &  0.976927 &  7542.857143 &  277.500000 &   0.088962 &  0.181294 &     0.017837 &      0.043984 &   0.025315 &     6634.747605 &  134.626779 \\      &       & int w halfs pace unn & pw 1 &  0.041954 &  0.044865 &  0.991832 &  0.983433 &  0.989514 &  7542.857143 &  277.500000 &   0.032931 &  0.057281 &     0.008782 &      0.019687 &   0.011384 &     6634.747605 &  134.626779 \\      &       & maha & pooled &  0.051324 &  0.054523 &  0.985813 &  0.985835 &  0.987170 &  7542.857143 &  277.500000 &   0.054251 &  0.110233 &     0.031747 &      0.029604 &   0.025798 &     6634.747605 &  134.626779 \\      &       & msp & softmax predictions &  0.104489 &  0.161952 &  0.970328 &  0.968133 &  0.969068 &  7542.857143 &  277.500000 &   0.037557 &  0.076477 &     0.013189 &      0.014757 &   0.013908 &     6634.747605 &  134.626779 \\      & trec & energy & energy predictions &  0.091820 &  0.257143 &  0.974788 &  0.841751 &  0.927795 &  7542.857143 &  277.500000 &   0.030335 &  0.143927 &     0.016948 &      0.091986 &   0.042511 &     6634.747605 &  134.626779 \\      &       & int w halfs pace unn & pw 1 &  0.045671 &  0.099800 &  0.995580 &  0.925654 &  0.982805 &  7542.857143 &  277.500000 &   0.040336 &  0.132692 &     0.005474 &      0.086669 &   0.020951 &     6634.747605 &  134.626779 \\      &       & maha & pooled &  0.071876 &  0.165000 &  0.986465 &  0.894089 &  0.961943 &  7542.857143 &  277.500000 &   0.042028 &  0.195857 &     0.026021 &      0.131033 &   0.057553 &     6634.747605 &  134.626779 \\      &       & msp & softmax predictions &  0.117005 &  0.376429 &  0.964148 &  0.775631 &  0.894399 &  7542.857143 &  277.500000 &   0.033103 &  0.157559 &     0.019951 &      0.102672 &   0.054313 &     6634.747605 &  134.626779 \\      & wmt16 & energy & energy predictions &  0.176778 &  0.257300 &  0.906070 &  0.960879 &  0.940582 &  7542.857143 &  277.500000 &   0.082122 &  0.133977 &     0.031246 &      0.020745 &   0.022215 &     6634.747605 &  134.626779 \\      &       & int w halfs pace unn & pw 1 &  0.067141 &  0.084219 &  0.981468 &  0.987347 &  0.984306 &  7542.857143 &  277.500000 &   0.068351 &  0.106556 &     0.021396 &      0.014638 &   0.017954 &     6634.747605 &  134.626779 \\      &       & maha & pooled &  0.100336 &  0.132611 &  0.944217 &  0.977308 &  0.964746 &  7542.857143 &  277.500000 &   0.090340 &  0.147394 &     0.115269 &      0.038322 &   0.066399 &     6634.747605 &  134.626779 \\      &       & msp & softmax predictions &  0.261293 &  0.395246 &  0.864263 &  0.938812 &  0.906944 &  7542.857143 &  277.500000 &   0.070577 &  0.115211 &     0.035636 &      0.018658 &   0.027195 &     6634.747605 &  134.626779 \\ imdb & 20ng & energy & energy predictions &  0.093471 &  0.672792 &  0.989348 &  0.310453 &  0.876925 &  7100.000000 &  260.057143 &   0.014989 &  0.217415 &     0.007232 &      0.137346 &   0.072241 &     6456.431464 &  128.012441 \\      &       & int w halfs pace unn & pw 1 &  0.060233 &  0.196911 &  0.997302 &  0.697529 &  0.966300 &  7100.000000 &  260.057143 &   0.008966 &  0.126358 &     0.001630 &      0.132767 &   0.019625 &     6456.431464 &  128.012441 \\      &       & maha & pooled &  0.057826 &  0.165966 &  0.991361 &  0.780756 &  0.950692 &  7100.000000 &  260.057143 &   0.010720 &  0.148931 &     0.017399 &      0.149339 &   0.068617 &     6456.431464 &  128.012441 \\      &       & msp & softmax predictions &  0.089393 &  0.609803 &  0.991019 &  0.333099 &  0.894307 &  7100.000000 &  260.057143 &   0.012045 &  0.171112 &     0.005174 &      0.104325 &   0.051336 &     6456.431464 &  128.012441 \\      & mnli & energy & energy predictions &  0.323172 &  0.670863 &  0.927849 &  0.795123 &  0.886550 &  7100.000000 &  260.057143 &   0.081700 &  0.185684 &     0.035428 &      0.094020 &   0.056569 &     6456.431464 &  128.012441 \\      &       & int w halfs pace unn & pw 1 &  0.057725 &  0.067630 &  0.992169 &  0.982312 &  0.988439 &  7100.000000 &  260.057143 &   0.045057 &  0.102364 &     0.008222 &      0.020349 &   0.012797 &     6456.431464 &  128.012441 \\      &       & maha & pooled &  0.090539 &  0.142211 &  0.935530 &  0.953051 &  0.945985 &  7100.000000 &  260.057143 &   0.057176 &  0.129917 &     0.115383 &      0.064320 &   0.092240 &     6456.431464 &  128.012441 \\      &       & msp & softmax predictions &  0.300021 &  0.618237 &  0.937068 &  0.825886 &  0.902083 &  7100.000000 &  260.057143 &   0.047456 &  0.107852 &     0.018438 &      0.042847 &   0.027301 &     6456.431464 &  128.012441 \\      & multi30k & energy & energy predictions &  0.098972 &  0.585996 &  0.990765 &  0.434702 &  0.911236 &  7100.000000 &  260.057143 &   0.030026 &  0.328541 &     0.008073 &      0.195051 &   0.070885 &     6456.431464 &  128.012441 \\      &       & int w halfs pace unn & pw 1 &  0.043109 &  0.007470 &  0.999809 &  0.979751 &  0.998085 &  7100.000000 &  260.057143 &   0.004470 &  0.023073 &     0.000418 &      0.037321 &   0.004155 &     6456.431464 &  128.012441 \\      &       & maha & pooled &  0.052440 &  0.088044 &  0.989882 &  0.897034 &  0.960004 &  7100.000000 &  260.057143 &   0.015363 &  0.161903 &     0.027696 &      0.163836 &   0.096633 &     6456.431464 &  128.012441 \\      &       & msp & softmax predictions &  0.085018 &  0.431319 &  0.994238 &  0.521960 &  0.943179 &  7100.000000 &  260.057143 &   0.019254 &  0.209140 &     0.002667 &      0.124973 &   0.025354 &     6456.431464 &  128.012441 \\      & rte & energy & energy predictions &  0.112785 &  0.636867 &  0.988345 &  0.446500 &  0.906167 &  7100.000000 &  260.057143 &   0.022059 &  0.206574 &     0.006687 &      0.137493 &   0.049235 &     6456.431464 &  128.012441 \\      &       & int w halfs pace unn & pw 1 &  0.050929 &  0.064571 &  0.998697 &  0.922054 &  0.989370 &  7100.000000 &  260.057143 &   0.012390 &  0.112693 &     0.001742 &      0.100689 &   0.014227 &     6456.431464 &  128.012441 \\      &       & maha & pooled &  0.053887 &  0.094043 &  0.986225 &  0.908833 &  0.956832 &  7100.000000 &  260.057143 &   0.015010 &  0.135881 &     0.033105 &      0.127553 &   0.094957 &     6456.431464 &  128.012441 \\      &       & msp & softmax predictions &  0.106423 &  0.576967 &  0.990101 &  0.469868 &  0.919502 &  7100.000000 &  260.057143 &   0.014455 &  0.134961 &     0.003278 &      0.080479 &   0.024664 &     6456.431464 &  128.012441 \\      & sst2 & energy & energy predictions &  0.105374 &  0.870895 &  0.972067 &  0.152341 &  0.724898 &  7100.000000 &  260.057143 &   0.006927 &  0.103864 &     0.007851 &      0.080930 &   0.064115 &     6456.431464 &  128.012441 \\      &       & int w halfs pace unn & pw 1 &  0.059164 &  0.190868 &  0.997607 &  0.759587 &  0.968716 &  7100.000000 &  260.057143 &   0.015881 &  0.230111 &     0.002838 &      0.195253 &   0.036079 &     6456.431464 &  128.012441 \\      &       & maha & pooled &  0.079403 &  0.486538 &  0.978768 &  0.467099 &  0.845368 &  7100.000000 &  260.057143 &   0.013033 &  0.190694 &     0.019834 &      0.182009 &   0.083215 &     6456.431464 &  128.012441 \\      &       & msp & softmax predictions &  0.104331 &  0.853197 &  0.974394 &  0.149565 &  0.740907 &  7100.000000 &  260.057143 &   0.004195 &  0.062376 &     0.006253 &      0.044378 &   0.049253 &     6456.431464 &  128.012441 \\      & trec & energy & energy predictions &  0.057661 &  0.477686 &  0.998428 &  0.193237 &  0.927340 &  7100.000000 &  260.057143 &   0.006997 &  0.365185 &     0.001779 &      0.132350 &   0.072338 &     6456.431464 &  128.012441 \\      &       & int w halfs pace unn & pw 1 &  0.045740 &  0.003857 &  0.999961 &  0.908891 &  0.998036 &  7100.000000 &  260.057143 &   0.003709 &  0.013242 &     0.000095 &      0.142799 &   0.004701 &     6456.431464 &  128.012441 \\      &       & maha & pooled &  0.052141 &  0.211829 &  0.997801 &  0.554209 &  0.943231 &  7100.000000 &  260.057143 &   0.004887 &  0.209403 &     0.003972 &      0.302552 &   0.073424 &     6456.431464 &  128.012441 \\      &       & msp & softmax predictions &  0.054859 &  0.322543 &  0.999087 &  0.226913 &  0.955754 &  7100.000000 &  260.057143 &   0.005282 &  0.243224 &     0.000607 &      0.093189 &   0.027836 &     6456.431464 &  128.012441 \\      & wmt16 & energy & energy predictions &  0.107778 &  0.590211 &  0.988429 &  0.470602 &  0.907667 &  7100.000000 &  260.057143 &   0.026555 &  0.248399 &     0.008013 &      0.163710 &   0.058483 &     6456.431464 &  128.012441 \\      &       & int w halfs pace unn & pw 1 &  0.046652 &  0.031730 &  0.999314 &  0.954582 &  0.994276 &  7100.000000 &  260.057143 &   0.008064 &  0.068086 &     0.001113 &      0.068804 &   0.009277 &     6456.431464 &  128.012441 \\      &       & maha & pooled &  0.061411 &  0.159868 &  0.976987 &  0.851240 &  0.926090 &  7100.000000 &  260.057143 &   0.016817 &  0.155909 &     0.043113 &      0.147372 &   0.122141 &     6456.431464 &  128.012441 \\      &       & msp & softmax predictions &  0.100301 &  0.519926 &  0.990738 &  0.502521 &  0.925140 &  7100.000000 &  260.057143 &   0.016026 &  0.149643 &     0.003054 &      0.089347 &   0.023389 &     6456.431464 &  128.012441 \\ sst2 & 20ng & energy & energy predictions &  0.365704 &  0.669235 &  0.896322 &  0.810810 &  0.868381 &  8000.000000 &  277.500000 &   0.147490 &  0.289238 &     0.068364 &      0.102333 &   0.076053 &     6759.197215 &  124.847135 \\      &       & int w halfs pace unn & pw 1 &  0.053378 &  0.060428 &  0.992182 &  0.986896 &  0.990137 &  8000.000000 &  277.500000 &   0.059466 &  0.114409 &     0.011036 &      0.020586 &   0.014659 &     6759.197215 &  124.847135 \\      &       & maha & pooled &  0.196020 &  0.336510 &  0.903532 &  0.909307 &  0.912186 &  8000.000000 &  277.500000 &   0.122575 &  0.240120 &     0.114777 &      0.088728 &   0.092742 &     6759.197215 &  124.847135 \\      &       & msp & softmax predictions &  0.364439 &  0.666610 &  0.894812 &  0.819406 &  0.867615 &  8000.000000 &  277.500000 &   0.127424 &  0.249937 &     0.083854 &      0.093448 &   0.083335 &     6759.197215 &  124.847135 \\      & imdb & energy & energy predictions &  0.788227 &  0.842002 &  0.286912 &  0.959561 &  0.700508 &  8000.000000 &  277.500000 &   0.170547 &  0.182970 &     0.189185 &      0.016319 &   0.111836 &     6759.197215 &  124.847135 \\      &       & int w halfs pace unn & pw 1 &  0.376488 &  0.400307 &  0.603921 &  0.990294 &  0.907687 &  8000.000000 &  277.500000 &   0.217502 &  0.233285 &     0.178528 &      0.008924 &   0.070863 &     6759.197215 &  124.847135 \\      &       & maha & pooled &  0.723477 &  0.772537 &  0.202841 &  0.960563 &  0.697791 &  8000.000000 &  277.500000 &   0.228740 &  0.245401 &     0.130490 &      0.020889 &   0.122649 &     6759.197215 &  124.847135 \\      &       & msp & softmax predictions &  0.790962 &  0.844938 &  0.286936 &  0.961359 &  0.705674 &  8000.000000 &  277.500000 &   0.153498 &  0.164680 &     0.169459 &      0.015216 &   0.102476 &     6759.197215 &  124.847135 \\      & mnli & energy & energy predictions &  0.716467 &  0.778255 &  0.432670 &  0.967675 &  0.793627 &  8000.000000 &  277.500000 &   0.114326 &  0.124925 &     0.141405 &      0.013057 &   0.073824 &     6759.197215 &  124.847135 \\      &       & int w halfs pace unn & pw 1 &  0.408391 &  0.441622 &  0.664540 &  0.988246 &  0.909876 &  8000.000000 &  277.500000 &   0.160123 &  0.174965 &     0.109931 &      0.007456 &   0.043174 &     6759.197215 &  124.847135 \\      &       & maha & pooled &  0.427502 &  0.462502 &  0.433316 &  0.983037 &  0.854140 &  8000.000000 &  277.500000 &   0.102279 &  0.111762 &     0.180514 &      0.011602 &   0.093919 &     6759.197215 &  124.847135 \\      &       & msp & softmax predictions &  0.720528 &  0.782691 &  0.448121 &  0.967532 &  0.792318 &  8000.000000 &  277.500000 &   0.126651 &  0.138392 &     0.145861 &      0.013643 &   0.085510 &     6759.197215 &  124.847135 \\      & multi30k & energy & energy predictions &  0.466162 &  0.765643 &  0.800794 &  0.806190 &  0.811367 &  8000.000000 &  277.500000 &   0.099443 &  0.171100 &     0.112864 &      0.100673 &   0.103116 &     6759.197215 &  124.847135 \\      &       & int w halfs pace unn & pw 1 &  0.241451 &  0.379274 &  0.916364 &  0.924062 &  0.919321 &  8000.000000 &  277.500000 &   0.133765 &  0.230096 &     0.078512 &      0.080072 &   0.081897 &     6759.197215 &  124.847135 \\      &       & maha & pooled &  0.239093 &  0.375188 &  0.869981 &  0.918312 &  0.899696 &  8000.000000 &  277.500000 &   0.115825 &  0.199171 &     0.134355 &      0.078338 &   0.102716 &     6759.197215 &  124.847135 \\      &       & msp & softmax predictions &  0.463260 &  0.760584 &  0.817129 &  0.825898 &  0.827001 &  8000.000000 &  277.500000 &   0.053943 &  0.092809 &     0.085537 &      0.065598 &   0.074350 &     6759.197215 &  124.847135 \\      & rte & energy & energy predictions &  0.457018 &  0.704167 &  0.826179 &  0.868120 &  0.852958 &  8000.000000 &  277.500000 &   0.111887 &  0.179853 &     0.115344 &      0.057173 &   0.073775 &     6759.197215 &  124.847135 \\      &       & int w halfs pace unn & pw 1 &  0.093201 &  0.119885 &  0.974510 &  0.985122 &  0.980251 &  8000.000000 &  277.500000 &   0.073796 &  0.118184 &     0.019246 &      0.014952 &   0.016989 &     6759.197215 &  124.847135 \\      &       & maha & pooled &  0.145326 &  0.203313 &  0.865398 &  0.959294 &  0.926891 &  8000.000000 &  277.500000 &   0.098364 &  0.158070 &     0.172490 &      0.049598 &   0.094305 &     6759.197215 &  124.847135 \\      &       & msp & softmax predictions &  0.459204 &  0.707635 &  0.830956 &  0.867764 &  0.851749 &  8000.000000 &  277.500000 &   0.111069 &  0.178490 &     0.122445 &      0.066023 &   0.090209 &     6759.197215 &  124.847135 \\      & trec & energy & energy predictions &  0.209141 &  0.796952 &  0.949156 &  0.486042 &  0.825848 &  8000.000000 &  277.500000 &   0.031780 &  0.153855 &     0.034858 &      0.137510 &   0.092518 &     6759.197215 &  124.847135 \\      &       & int w halfs pace unn & pw 1 &  0.117442 &  0.364310 &  0.985190 &  0.758314 &  0.943422 &  8000.000000 &  277.500000 &   0.046969 &  0.218079 &     0.008182 &      0.110298 &   0.030636 &     6759.197215 &  124.847135 \\      &       & maha & pooled &  0.142765 &  0.483071 &  0.953878 &  0.677554 &  0.870391 &  8000.000000 &  277.500000 &   0.049616 &  0.230628 &     0.046856 &      0.179818 &   0.106586 &     6759.197215 &  124.847135 \\      &       & msp & softmax predictions &  0.202976 &  0.763786 &  0.954556 &  0.508335 &  0.839201 &  8000.000000 &  277.500000 &   0.033228 &  0.157357 &     0.030287 &      0.135722 &   0.087351 &     6759.197215 &  124.847135 \\      & wmt16 & energy & energy predictions &  0.503040 &  0.778204 &  0.752183 &  0.834491 &  0.803116 &  8000.000000 &  277.500000 &   0.076212 &  0.122496 &     0.100426 &      0.052106 &   0.069002 &     6759.197215 &  124.847135 \\      &       & int w halfs pace unn & pw 1 &  0.258239 &  0.384751 &  0.886172 &  0.942874 &  0.918129 &  8000.000000 &  277.500000 &   0.089750 &  0.144232 &     0.046001 &      0.030207 &   0.036570 &     6759.197215 &  124.847135 \\      &       & maha & pooled &  0.251198 &  0.373466 &  0.790728 &  0.929103 &  0.879037 &  8000.000000 &  277.500000 &   0.068317 &  0.109858 &     0.148317 &      0.046152 &   0.089490 &     6759.197215 &  124.847135 \\      &       & msp & softmax predictions &  0.505016 &  0.781376 &  0.756675 &  0.830623 &  0.801224 &  8000.000000 &  277.500000 &   0.085069 &  0.136749 &     0.108839 &      0.063795 &   0.084959 &     6759.197215 &  124.847135 \\ trec & 20ng & energy & energy predictions &  0.035684 &  0.032430 &  0.981803 &  0.997041 &  0.991613 &  7775.000000 &  274.725000 &   0.031257 &  0.039106 &     0.012994 &      0.002523 &   0.006163 &     6733.582942 &  127.327344 \\      &       & int w halfs pace unn & pw 1 &  0.014175 &  0.006784 &  0.989373 &  0.996666 &  0.993486 &  7775.000000 &  274.725000 &   0.011968 &  0.013891 &     0.007668 &      0.003647 &   0.005342 &     6733.582942 &  127.327344 \\      &       & maha & pooled &  0.010930 &  0.004503 &  0.993730 &  0.998652 &  0.996731 &  7775.000000 &  274.725000 &   0.009255 &  0.009287 &     0.006949 &      0.002362 &   0.004320 &     6733.582942 &  127.327344 \\      &       & msp & softmax predictions &  0.036451 &  0.033142 &  0.976634 &  0.994210 &  0.986565 &  7775.000000 &  274.725000 &   0.033730 &  0.042481 &     0.011901 &      0.004427 &   0.007548 &     6733.582942 &  127.327344 \\      & imdb & energy & energy predictions &  0.115736 &  0.117053 &  0.823119 &  0.999322 &  0.976959 &  7775.000000 &  274.725000 &   0.112682 &  0.114933 &     0.143933 &      0.000499 &   0.017699 &     6733.582942 &  127.327344 \\      &       & int w halfs pace unn & pw 1 &  0.089360 &  0.090161 &  0.914597 &  0.999224 &  0.980506 &  7775.000000 &  274.725000 &   0.127308 &  0.129845 &     0.064536 &      0.000742 &   0.016400 &     6733.582942 &  127.327344 \\      &       & maha & pooled &  0.024923 &  0.024467 &  0.945582 &  0.999725 &  0.991459 &  7775.000000 &  274.725000 &   0.045924 &  0.046819 &     0.060498 &      0.000277 &   0.008277 &     6733.582942 &  127.327344 \\      &       & msp & softmax predictions &  0.118347 &  0.119714 &  0.830045 &  0.999086 &  0.972624 &  7775.000000 &  274.725000 &   0.112121 &  0.114363 &     0.130898 &      0.000536 &   0.016133 &     6733.582942 &  127.327344 \\      & mnli & energy & energy predictions &  0.126898 &  0.128856 &  0.649246 &  0.999193 &  0.973384 &  7775.000000 &  274.725000 &   0.061380 &  0.062941 &     0.108220 &      0.000311 &   0.010000 &     6733.582942 &  127.327344 \\      &       & int w halfs pace unn & pw 1 &  0.112899 &  0.114501 &  0.776319 &  0.999018 &  0.975101 &  7775.000000 &  274.725000 &   0.076689 &  0.078640 &     0.074985 &      0.000570 &   0.011329 &     6733.582942 &  127.327344 \\      &       & maha & pooled &  0.037831 &  0.037526 &  0.834132 &  0.999692 &  0.989698 &  7775.000000 &  274.725000 &   0.031040 &  0.031826 &     0.088864 &      0.000210 &   0.006552 &     6733.582942 &  127.327344 \\      &       & msp & softmax predictions &  0.140933 &  0.143248 &  0.648765 &  0.998873 &  0.967296 &  7775.000000 &  274.725000 &   0.049233 &  0.050486 &     0.096106 &      0.000305 &   0.008369 &     6733.582942 &  127.327344 \\      & multi30k & energy & energy predictions &  0.290299 &  0.337776 &  0.819648 &  0.982512 &  0.932813 &  7775.000000 &  274.725000 &   0.170964 &  0.204708 &     0.131855 &      0.011748 &   0.046382 &     6733.582942 &  127.327344 \\      &       & int w halfs pace unn & pw 1 &  0.156155 &  0.177177 &  0.928409 &  0.989883 &  0.968960 &  7775.000000 &  274.725000 &   0.118265 &  0.141580 &     0.043679 &      0.007246 &   0.019727 &     6733.582942 &  127.327344 \\      &       & maha & pooled &  0.091532 &  0.099936 &  0.957137 &  0.995287 &  0.981940 &  7775.000000 &  274.725000 &   0.104800 &  0.125338 &     0.038092 &      0.004895 &   0.017556 &     6733.582942 &  127.327344 \\      &       & msp & softmax predictions &  0.319162 &  0.372339 &  0.800104 &  0.977162 &  0.920634 &  7775.000000 &  274.725000 &   0.186594 &  0.223456 &     0.150914 &      0.015671 &   0.056077 &     6733.582942 &  127.327344 \\      & rte & energy & energy predictions &  0.074479 &  0.078612 &  0.941982 &  0.997121 &  0.984895 &  7775.000000 &  274.725000 &   0.048626 &  0.056689 &     0.039105 &      0.001741 &   0.008872 &     6733.582942 &  127.327344 \\      &       & int w halfs pace unn & pw 1 &  0.043768 &  0.042946 &  0.969785 &  0.997218 &  0.988891 &  7775.000000 &  274.725000 &   0.036633 &  0.042534 &     0.017747 &      0.002418 &   0.007406 &     6733.582942 &  127.327344 \\      &       & maha & pooled &  0.017861 &  0.013137 &  0.983088 &  0.999170 &  0.995629 &  7775.000000 &  274.725000 &   0.015280 &  0.017367 &     0.020814 &      0.000730 &   0.003750 &     6733.582942 &  127.327344 \\      &       & msp & softmax predictions &  0.094039 &  0.101412 &  0.932410 &  0.994840 &  0.976969 &  7775.000000 &  274.725000 &   0.047692 &  0.055640 &     0.034491 &      0.002067 &   0.009083 &     6733.582942 &  127.327344 \\      & sst2 & energy & energy predictions &  0.240134 &  0.292387 &  0.854043 &  0.978920 &  0.939003 &  7775.000000 &  274.725000 &   0.109380 &  0.139405 &     0.105273 &      0.011742 &   0.038784 &     6733.582942 &  127.327344 \\      &       & int w halfs pace unn & pw 1 &  0.287559 &  0.352828 &  0.891923 &  0.972631 &  0.940661 &  7775.000000 &  274.725000 &   0.153130 &  0.195160 &     0.062218 &      0.015554 &   0.031918 &     6733.582942 &  127.327344 \\      &       & maha & pooled &  0.091970 &  0.103734 &  0.953033 &  0.992573 &  0.979202 &  7775.000000 &  274.725000 &   0.075057 &  0.095477 &     0.040625 &      0.005309 &   0.015164 &     6733.582942 &  127.327344 \\      &       & msp & softmax predictions &  0.247366 &  0.301627 &  0.859889 &  0.976901 &  0.938415 &  7775.000000 &  274.725000 &   0.098411 &  0.125452 &     0.098033 &      0.010161 &   0.032055 &     6733.582942 &  127.327344 \\      & wmt16 & energy & energy predictions &  0.088379 &  0.094802 &  0.918956 &  0.996463 &  0.981024 &  7775.000000 &  274.725000 &   0.043036 &  0.050189 &     0.038185 &      0.001541 &   0.008039 &     6733.582942 &  127.327344 \\      &       & int w halfs pace unn & pw 1 &  0.068791 &  0.071978 &  0.952379 &  0.995545 &  0.982816 &  7775.000000 &  274.725000 &   0.047427 &  0.055295 &     0.021494 &      0.002901 &   0.008733 &     6733.582942 &  127.327344 \\      &       & maha & pooled &  0.025386 &  0.021520 &  0.975334 &  0.998870 &  0.993953 &  7775.000000 &  274.725000 &   0.019023 &  0.022040 &     0.017509 &      0.000864 &   0.004466 &     6733.582942 &  127.327344 \\      &       & msp & softmax predictions &  0.105473 &  0.114763 &  0.910937 &  0.994342 &  0.973853 &  7775.000000 &  274.725000 &   0.039900 &  0.046556 &     0.033726 &      0.001745 &   0.007797 &     6733.582942 &  127.327344 \\ \bottomrule 
\end{longtable}
